Stochastic Online Metric Matching

We study the minimum-cost metric perfect matching problem under online i.i.d arrivals. We are given a fixed metric with a server at each of the points, and then requests arrive online, each drawn independently from a known probability distribution over the points. Each request has to be matched to a free server, with cost equal to the distance. The goal is to minimize the expected total cost of the matching. Such stochastic arrival models have been widely studied for the maximization variants of the online matching problem; however, the only known result for the minimization problem is a tight $O(\log n)$-competitiveness for the random-order arrival model. This is in contrast with the adversarial model, where an optimal competitive ratio of $O(\log n)$ has long been conjectured and remains a tantalizing open question. In this paper, we show improved results in the i.i.d arrival model. We show how the i.i.d model can be used to give substantially better algorithms: our main result is an $O((\log \log \log n)^2)$-competitive algorithm in this model. Along the way we give a $9$-competitive algorithm for the line and tree metrics. Both results imply a strict separation between the i.i.d model and the adversarial and random order models, both for general metrics and these much-studied metrics.

==> tree-algo.tex <==
\section{An Alternative Algorithm for Tree Metrics}\bpnote{Do we need to
  write down this in our paper?} \agnote{Eventually yes, but I am not
  sure it should go in right now.}
\subsection{Tree Metric}
Though lemma 1 applies for general metric, in the following, we focus on tree metric and we give a $O(1)$ competitive algorithm. Formally, we will use $T$ to denote the tree spanned by all servers, and we assume servers are represented by leaves of the tree. The distance between any two node is just the shortest path distance. We use $n$ to denote the number of servers
\begin{obs}
	We can assume the maximum degree of the tree is 3 by adding $O(n)$ edge to tree with 0 cost
\end{obs}

\noindent Next, we are going to recursively split $T$ into two parts of roughly same size(say 1/3 versus 2/3n) and mark the edge with its corresponding level. Formally, the algorithm is shown in \autoref{alg:matching}

\subsubsection{Notation}
Before going on, we define some notation here. For each tree edge $e$, we use $T_e$ to denote the size of its smaller subtree. A bit abuse of notation, we will also use $T_e$ to denote the smaller subtree. We use $X_e$ to denote the number of requests arrives in $T_e$, $l_e$ to denote the length $e$.\\
Let $T_e^{k}$ denote subtree of $e$ in level $k$(notice that $T_e^k$ may not necessary be same as $T_e$) and $\widetilde{T^{k}_e}$ denote the subtree contains $e$ in level $k$. Also, sometimes we will use $T_e^{k}$ and$\widetilde{T^{k}_e}$ to refer the size of tree. Finally, let $k_e$ be the smallest marked edge in $T_e$.
\subsubsection{Algorithm}
We describes the algorithm in \autoref{alg:matching}, 
\begin{algorithm}[h] 
	\caption{Matching algorithm}
	\label{alg:matching}
	\begin{algorithmic}
	\Function{Split}{$k, T$}
	\State If there is only one edge $e$ in $T$, mark $e$ with $k$.
	\State Otherwise, find edge $e \in T$($e$ split $T$ into $T_0$, $T_1$), such that $|T_1|, |T_2| \leq 2/3|T|$.
	\State Mark $e$ with $k$ and call \Call{Split}{$k+1, T_0$}, \Call{Split}{$k + 1, T_1$}  
	\EndFunction

	\Function{Match}{$u$}
	\State If server in $u$ is vacant, just match to $u$.
	\State Otherwise, find edge $e$ with smallest $k$, such that $T_{ei}$($i \in \{0, 1\}$) contains $u$ and $T_{ei}$ is full, then uniform randomly select one leaf $v$ of $T_{e(1-i)}$, call \Call{Match}{$v$}
	\EndFunction
	\\
	\State Main algorithm:
	\State \Call{Split}{1, $T$}
	\Event{arrival of $r$}
	\State \Call{Match}{$r$}
	\EndEvent
	\end{algorithmic}
\end{algorithm}

To analyses the competitive ratio, we first give a lower bound for optimal matching
\begin{lem}(Lower Bound for OPT)
	$$E[OPT] = \sum_{e \in T}l_e E\left[\left|X_e - T_e\right|\right]$$
	Moreover, as $X_e \sim B(n, p)$ with $p = \frac{T_e}{n}$, we have
	$$E[OPT] \sim \Theta(\sum_{e \in T}l_e \sqrt{T_e})$$ 
\end{lem}
\begin{proof}
	To be writen.
\end{proof}
Let $N_e$ be the expected number of times $e$ was tranversed, and $N_e^{k}$ to denote the expected number of times $e$ was tranversed in level $k$, we have the following observation:
\begin{obs}
$$E[ALG] \leq \sum_{e}l_e N_e = \sum_{e} l_e \sum_{k}N_{e}^{k}$$
\end{obs}

The following lemma characterize $T_e^{k}$ and $\widetilde{T^{k}_e}$
\begin{lem}
	(Bound for Subtree Size)
	For any $e \in T$
	\begin{enumerate}
		\item for $k < k_e$, $T_e^{k} = T_e$
		\item $T^{k}_e \leq \widetilde{T^{k}_e} \leq \frac{2}{3} \widetilde{T^{k - 1}_e}$
		\item $\frac{1}{3}T_e \leq \widetilde{T^{k_e}_e} \leq 3T_e$
	\end{enumerate} 
\end{lem}
\begin{proof}
	To be writen.
\end{proof}
The following lemma gives a bound to $N_e^{k}$
\begin{lem}
	('Variance' Bound for each Level )
	For $\forall e \in T$, 
	$$N_e^k \leq \frac{T_e^{k}}{\sqrt{\widetilde{T_{e}^{k}}}}$$
\end{lem}
\begin{proof}
	To be writen
\end{proof}

\begin{thm}
	The algorithm is constant competitive for tree metric.
\end{thm}
\begin{proof}
	For each $e \in T$, we have
	\begin{align*}
	\sum_{k = 1}^{k_e - 1}N_e^{k} &\leq \sum_{k = 1}^{k_e - 1}\frac{T_e^{k}}{\sqrt{\widetilde{T_{e}^{k}}}}\\
	&=\sum_{k = 1}^{k_e - 1}\frac{T_e}{\sqrt{\widetilde{T_{e}^{k_e - 1}}}} \sqrt{\frac{\widetilde{T_e^{k_e - 1} }}{\widetilde{T_{e}^{k}}}}\\
	&\leq \sum_{k = 1}^{k_e - 1}\sqrt{T_e}(\frac{2}{3})^k\\
	&\leq \sqrt{T_e}
	\end{align*}
	\begin{align*}
	\sum_{k = k_e}N_e^{k} &\leq \sum_{k = 1}^{k_e - 1}\frac{T_e^{k}}{\sqrt{\widetilde{T_{e}^{k}}}}\\
	&\leq\sum_{k = k_e}\sqrt{\widetilde{T_{e}^{k}}}\\
	&\leq \sqrt{T_e} \sum_{k_e}(\frac{2}{3})^k\\
	&\leq \sqrt{T_e}
	\end{align*}
In summary, 
$$E[ALG] \leq \sum_{e} l_e \sum_{k}N_{e}^{k} \leq\sum_{e} l_e (\sum_{k^e - 1}N_{e}^{k} + \sum_{k_e}N_{e}^{k_e - 1}) \leq \sum_{e} l_e\sqrt{T_e} \leq E[OPT]$$
\end{proof}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

